Probing Higgs self-coupling of a classically scale invariant model in $e^+e^- \to Zhh$: Evaluation at physical point

A classically scale invariant extension of the standard model predicts large anomalous Higgs self-interactions. We compute missing contributions in previous studies for probing the Higgs triple coupling of a minimal model using the process $e^+e^- \to Zhh$. Employing a proper order counting, we compute the total and differential cross sections at the leading order, which incorporate the one-loop corrections between zero external momenta and their physical values. Discovery/exclusion potential of a future $e^+e^-$ collider for this model is estimated. We also find a unique feature in the momentum dependence of the Higgs triple vertex for this class of models.

==> refs.tex <==


\begin{thebibliography}{99}

%% inspire LaTeX(US)
%% %``->``
%% doi: -> %doi:
%% ," -> ",

%\cite{Aaboud:2017sjh}
\bibitem{Aaboud:2017sjh} 
  M.~Aaboud {\it et al.} [ATLAS Collaboration],
  ``Search for additional heavy neutral Higgs and gauge bosons in the ditau final state produced in 36 fb$^{-1}$ of $pp$ collisions at $\sqrt{s}$ = 13 TeV with the ATLAS detector'',
  [arXiv:1709.07242 [hep-ex]].
  %%CITATION = ARXIV:1709.07242;%%
  
  %\cite{Khachatryan:2014qaa}
\bibitem{Khachatryan:2014qaa} 
  V.~Khachatryan {\it et al.} [CMS Collaboration],
  ``Search for the associated production of the Higgs boson with a top-quark pair'',
  JHEP {\bf 1409}, 087 (2014),
 % Erratum: [JHEP {\bf 1410}, 106 (2014)]
  %doi:10.1007/JHEP09(2014)087, 10.1007/JHEP10(2014)106
  [arXiv:1408.1682 [hep-ex]].
  %%CITATION = %doi:10.1007/JHEP09(2014)087, 10.1007/JHEP10(2014)106;%%
  %167 citations counted in INSPIRE as of 16 Oct 2017
  
  %\cite{Aad:2015iha}
\bibitem{Aad:2015iha} 
  G.~Aad {\it et al.} [ATLAS Collaboration],
  ``Search for the associated production of the Higgs boson with a top quark pair in multilepton final states with the ATLAS detector'',
  Phys.\ Lett.\ B {\bf 749}, 519 (2015),
  %doi:10.1016/j.physletb.2015.07.079
  [arXiv:1506.05988 [hep-ex]].
  %%CITATION = %doi:10.1016/j.physletb.2015.07.079;%%
  %78 citations counted in INSPIRE as of 16 Oct 2017
  
  %\cite{CMS:2017vru}
\bibitem{CMS:2017vru} 
  CMS Collaboration [CMS Collaboration],
  ``Search for Higgs boson production in association with top quarks in multilepton final states at $\sqrt{s}=13~\mathrm{TeV}$'',
  CMS-PAS-HIG-17-004.
  %%CITATION = CMS-PAS-HIG-17-004;%%
  %15 citations counted in INSPIRE as of 16 Oct 2017
  
  %%%%%%%%%%%%5%%%%%%%%%%%
  
  %\cite{Coleman:1973jx}
\bibitem{Coleman:1973jx} 
  S.~R.~Coleman and E.~J.~Weinberg,
  ``Radiative Corrections as the Origin of Spontaneous Symmetry Breaking'',
  Phys.\ Rev.\ D {\bf 7}, 1888 (1973).
  %doi:10.1103/PhysRevD.7.1888
  %%CITATION = %doi:10.1103/PhysRevD.7.1888;%%
  %3943 citations counted in INSPIRE as of 16 Oct 2017
  
  %\cite{Burgess:2000yq}
\bibitem{Burgess:2000yq} 
  C.~P.~Burgess, M.~Pospelov and T.~ter Veldhuis,
  ``The Minimal model of nonbaryonic dark matter: A Singlet scalar'',
  Nucl.\ Phys.\ B {\bf 619}, 709 (2001),
  %doi:10.1016/S0550-3213(01)00513-2
  [hep-ph/0011335].
  %%CITATION = %doi:10.1016/S0550-3213(01)00513-2;%%
  %634 citations counted in INSPIRE as of 16 Oct 2017
  
  %\cite{Ghosh:2017fmr}
\bibitem{Ghosh:2017fmr} 
  P.~Ghosh, A.~K.~Saha and A.~Sil,
  ``Study of Electroweak Vacuum Stability from Extended Higgs Portal of Dark Matter and Neutrinos'',
  arXiv:1706.04931 [hep-ph].
  %%CITATION = ARXIV:1706.04931;%%
  %2 citations counted in INSPIRE as of 16 Oct 2017
  
  %\cite{Silveira:1985rk}
\bibitem{Silveira:1985rk} 
  V.~Silveira and A.~Zee,
  ``Scalar Phantoms'',
  Phys.\ Lett.\  {\bf 161B}, 136 (1985).
  %doi:10.1016/0370-2693(85)90624-0
  %%CITATION = %doi:10.1016/0370-2693(85)90624-0;%%
  %446 citations counted in INSPIRE as of 16 Oct 2017
  
 %\cite{McDonald:1993ex}
\bibitem{McDonald:1993ex} 
  J.~McDonald,
  ``Gauge singlet scalars as cold dark matter'',
  Phys.\ Rev.\ D {\bf 50}, 3637 (1994),
  %doi:10.1103/PhysRevD.50.3637
  [hep-ph/0702143 [HEP-PH]].
  %%CITATION = %doi:10.1103/PhysRevD.50.3637;%%
  %564 citations counted in INSPIRE as of 16 Oct 2017
  
  %%%%%%%%10%%%%%%%
  
  %\cite{Cline:2013gha}
\bibitem{Cline:2013gha} 
  J.~M.~Cline, K.~Kainulainen, P.~Scott and C.~Weniger,
  ``Update on scalar singlet dark matter'',
  Phys.\ Rev.\ D {\bf 88}, 055025 (2013),
%  Erratum: [Phys.\ Rev.\ D {\bf 92}, no. 3, 039906 (2015)]
  %doi:10.1103/PhysRevD.92.039906, 10.1103/PhysRevD.88.055025
  [arXiv:1306.4710 [hep-ph]].
  %%CITATION = %doi:10.1103/PhysRevD.92.039906, 10.1103/PhysRevD.88.055025;%%
  %270 citations counted in INSPIRE as of 16 Oct 2017
  
  %\cite{Guo:2010hq}
\bibitem{Guo:2010hq} 
  W.~L.~Guo and Y.~L.~Wu,
  ``The Real singlet scalar dark matter model'',
  JHEP {\bf 1010}, 083 (2010),
  %doi:10.1007/JHEP10(2010)083
  [arXiv:1006.2518 [hep-ph]].
  %%CITATION = %doi:10.1007/JHEP10(2010)083;%%
  %76 citations counted in INSPIRE as of 16 Oct 2017
  
  %\cite{Endo:2015nba}
\bibitem{Endo:2015nba} 
  K.~Endo and K.~Ishiwata,
  ``Direct detection of singlet dark matter in classically scale-invariant standard model,''
  Phys.\ Lett.\ B {\bf 749}, 583 (2015)
  %doi:10.1016/j.physletb.2015.08.059
  [arXiv:1507.01739 [hep-ph]].
  %%CITATION = doi:10.1016/j.physletb.2015.08.059;%%
  %11 citations counted in INSPIRE as of 16 Oct 2017
  
  
  %%  %\cite{Ishiwata:2011aa}
\bibitem{Ishiwata:2011aa} 
  K.~Ishiwata,
  %``Dark Matter in Classically Scale-Invariant Two Singlets Standard Model,''
  Phys.\ Lett.\ B {\bf 710}, 134 (2012)
  doi:10.1016/j.physletb.2012.02.048
  [arXiv:1112.2696 [hep-ph]].
  %%CITATION = doi:10.1016/j.physletb.2012.02.048;%%
  %40 citations counted in INSPIRE as of 25 Oct 2017

%\cite{Heikinheimo:2013fta}
\bibitem{Heikinheimo:2013fta} 
  M.~Heikinheimo, A.~Racioppi, M.~Raidal, C.~Spethmann and K.~Tuominen,
  ``Physical Naturalness and Dynamical Breaking of Classical Scale Invariance,''
  Mod.\ Phys.\ Lett.\ A {\bf 29}, 1450077 (2014)
  %doi:10.1142/S0217732314500771
  [arXiv:1304.7006 [hep-ph]].
  %%CITATION = doi:10.1142/S0217732314500771;%%
  %131 citations counted in INSPIRE as of 25 Oct 2017

%\cite{Gabrielli:2013hma}
\bibitem{Gabrielli:2013hma} 
  E.~Gabrielli, M.~Heikinheimo, K.~Kannike, A.~Racioppi, M.~Raidal and C.~Spethmann,
  ``Towards Completing the Standard Model: Vacuum Stability, EWSB and Dark Matter,''
  Phys.\ Rev.\ D {\bf 89}, no. 1, 015017 (2014)
  %doi:10.1103/PhysRevD.89.015017
  [arXiv:1309.6632 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevD.89.015017;%%
  %108 citations counted in INSPIRE as of 25 Oct 2017

%\cite{Davoudiasl:2014pya}
\bibitem{Davoudiasl:2014pya} 
H.~Davoudiasl and I.~M.~Lewis,
``Right-Handed Neutrinos as the Origin of the Electroweak Scale,''
  Phys.\ Rev.\ D {\bf 90}, no. 3, 033003 (2014)
  %doi:10.1103/PhysRevD.90.033003
  [arXiv:1404.6260 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevD.90.033003;%%

  
  %\cite{Dermisek:2013pta}
\bibitem{Dermisek:2013pta} 
  D.~Chway, T.~H.~Jung, H.~D.~Kim and R.~Dermisek,
  ``Radiative Electroweak Symmetry Breaking Model Perturbative All the Way to the Planck Scale'',
  Phys.\ Rev.\ Lett.\  {\bf 113}, no. 5, 051801 (2014),
  %doi:10.1103/PhysRevLett.113.051801
  [arXiv:1308.0891 [hep-ph]].
  %%CITATION = %doi:10.1103/PhysRevLett.113.051801;%%
  %39 citations counted in INSPIRE as of 16 Oct 2017
  
  %\cite{Endo:2015ifa}
\bibitem{Endo:2015ifa} 
  K.~Endo and Y.~Sumino,
  ``A Scale-invariant Higgs Sector and Structure of the Vacuum'',
  JHEP {\bf 1505}, 030 (2015),
  %doi:10.1007/JHEP05(2015)030
  [arXiv:1503.02819 [hep-ph]].
  %%CITATION = %doi:10.1007/JHEP05(2015)030;%%
  %19 citations counted in INSPIRE as of 16 Oct 2017
  
  %\cite{Hashino:2015nxa}
\bibitem{Hashino:2015nxa} 
  K.~Hashino, S.~Kanemura and Y.~Orikasa,
  ``Discriminative phenomenological features of scale invariant models for electroweak symmetry breaking'',
  Phys.\ Lett.\ B {\bf 752}, 217 (2016),
  %doi:10.1016/j.physletb.2015.11.044
  [arXiv:1508.03245 [hep-ph]].
  %%CITATION = %doi:10.1016/j.physletb.2015.11.044;%%
  %15 citations counted in INSPIRE as of 16 Oct 2017
  
  %\cite{Gounaris:1979px}
\bibitem{Gounaris:1979px} 
  G.~J.~Gounaris, D.~Schildknecht and F.~M.~Renard,
  %``Test of Higgs Boson Nature in $e^+ e^- \to H H Z$,''
  Phys.\ Lett.\  {\bf 83B}, 191 (1979).
  doi:10.1016/0370-2693(79)90683-X
  %%CITATION = doi:10.1016/0370-2693(79)90683-X;%%
  %73 citations counted in INSPIRE as of 12 Nov 2017
  
  %\cite{Barklow:2017awn}
\bibitem{Barklow:2017awn} 
  T.~Barklow, K.~Fujii, S.~Jung, M.~E.~Peskin and J.~Tian,
  ``Model-Independent Determination of the Triple Higgs Coupling at e+e- Colliders'',
  [arXiv:1708.09079 [hep-ph]].
  %%CITATION = ARXIV:1708.09079;%%
  %4 citations counted in INSPIRE as of 16 Oct 2017
  
  %\cite{Endo:2016koi}
\bibitem{Endo:2016koi} 
  K.~Endo, K.~Ishiwata and Y.~Sumino,
  ``$WW$ scattering in a radiative electroweak symmetry breaking scenario'',
  Phys.\ Rev.\ D {\bf 94}, no. 7, 075007 (2016),
  %doi:10.1103/PhysRevD.94.075007
  [arXiv:1601.00696 [hep-ph]].
  %%CITATION = %doi:10.1103/PhysRevD.94.075007;%%
  %3 citations counted in INSPIRE as of 16 Oct 2017
  
  %\cite{McKay:2017iur}
\bibitem{McKay:2017iur} 
  J.~McKay [GAMBIT Collaboration],
  ``Global fits of the scalar singlet model using GAMBIT'',
  [arXiv:1710.02467 [hep-ph]].
  %%CITATION = ARXIV:1710.02467;%%
  
  %\cite{Aprile:2017iyp}
\bibitem{Aprile:2017iyp} 
  E.~Aprile {\it et al.} [XENON Collaboration],
  ``First Dark Matter Search Results from the XENON1T Experiment'',
  [arXiv:1705.06655 [astro-ph.CO]].
  %%CITATION = ARXIV:1705.06655;%%
  %107 citations counted in INSPIRE as of 16 Oct 2017
  
  %\cite{Aad:2014aba}
\bibitem{Aad:2014aba} 
  G.~Aad {\it et al.} [ATLAS Collaboration],
  ``Measurement of the Higgs boson mass from the $H\rightarrow \gamma\gamma$ and $H \rightarrow ZZ^{*} \rightarrow 4\ell$ channels with the ATLAS detector using 25 fb$^{-1}$ of $pp$ collision data'',
  Phys.\ Rev.\ D {\bf 90}, no. 5, 052004 (2014),
  %doi:10.1103/PhysRevD.90.052004
  [arXiv:1406.3827 [hep-ex]].
  %%CITATION = %doi:10.1103/PhysRevD.90.052004;%%
  %377 citations counted in INSPIRE as of 16 Oct 2017
  
  %\cite{Khachatryan:2014ira}
\bibitem{Khachatryan:2014ira} 
  V.~Khachatryan {\it et al.} [CMS Collaboration],
  ``Observation of the diphoton decay of the Higgs boson and measurement of its properties'',
  Eur.\ Phys.\ J.\ C {\bf 74}, no. 10, 3076 (2014),
  %doi:10.1140/epjc/s10052-014-3076-z
  [arXiv:1407.0558 [hep-ex]].
  %%CITATION = %doi:10.1140/epjc/s10052-014-3076-z;%%
  %382 citations counted in INSPIRE as of 16 Oct 2017
  
  %\cite{ATLAS:2014wva}
\bibitem{ATLAS:2014wva} 
  [ATLAS and CDF and CMS and D0 Collaborations],
  ``First combination of Tevatron and LHC measurements of the top-quark mass'',
  arXiv:1403.4427 [hep-ex].
  %%CITATION = ARXIV:1403.4427;%%
  %492 citations counted in INSPIRE as of 16 Oct 2017
  
%\cite{Alwall:2014hca}
\bibitem{Alwall:2014hca} 
  J.~Alwall {\it et al.},
  ``The automated computation of tree-level and next-to-leading order differential cross sections, and their matching to parton shower simulations'',
  JHEP {\bf 1407}, 079 (2014),
  %doi:10.1007/JHEP07(2014)079
  [arXiv:1405.0301 [hep-ph]].
  %%CITATION = %doi:10.1007/JHEP07(2014)079;%%
  %2224 citations counted in INSPIRE as of 16 Oct 2017
  
  %\cite{Tian:2013qmi}
\bibitem{Tian:2013qmi} 
  J.~Tian,
  ``Study of Higgs self-coupling at the ILC based on the full detector simulation at $\sqrt{s} = 500$ GeV and $\sqrt{s} = 1$ TeV'',
  %%CITATION = INSPIRE-1475534;%%
  %1 citations counted in INSPIRE as of 16 Oct 2017
  
  %\cite{Tian:2013yda}
\bibitem{Tian:2013yda} 
  J.~Tian {\it et al.} [ILD Collaboration],
  ``Measurement of Higgs couplings and self-coupling at the ILC'',
  PoS EPS {\bf -HEP2013}, 316 (2013),
  [arXiv:1311.6528 [hep-ph]].
  %%CITATION = ARXIV:1311.6528;%%
  %18 citations counted in INSPIRE as of 16 Oct 2017
  
  

  
  
  
  \end{thebibliography}
  
  
  
  
  
  
  
  
